A Solvable High-Dimensional Model of GAN

We present a theoretical analysis of the training process for a single-layer GAN fed by high-dimensional input data. The training dynamics of the proposed model at both microscopic and macroscopic scales can be exactly analyzed in the high-dimensional limit. In particular, we prove that the macroscopic quantities measuring the quality of the training process converge to a deterministic process characterized by an ordinary differential equation (ODE), whereas the microscopic states containing all the detailed weights remain stochastic, whose dynamics can be described by a stochastic differential equation (SDE). This analysis provides a new perspective different from recent analyses in the limit of small learning rate, where the microscopic state is always considered deterministic, and the contribution of noise is ignored. From our analysis, we show that the level of the background noise is essential to the convergence of the training process: setting the noise level too strong leads to failure of feature recovery, whereas setting the noise too weak causes oscillation. Although this work focuses on a simple copy model of GAN, we believe the analysis methods and insights developed here would prove useful in the theoretical understanding of other variants of GANs with more advanced training algorithms.

==> phase.tex <==
\subsection{Phase diagram and oscillation in $d=1 $ case}
%What happens when the left inequality in \eqref{eq:con} does hold, i.e. when noise is too weak or $\a=\tau/\tau$ is too large? To have a better understanding, it's better to study an even simple case when $d=1$. In this case, we are able to compute all the possible fixed points of the ODE, and fully characterized their local stability.

In what follows, we provide a thorough study of all the fixed points of the ODE \eqref{eq:PCA-ODE} when the number of feature $d=1$.  For simplicity, we only present the result when $\eta_{\text{T}}=\eta_{\text{G}}=1$, and $ \mat\Lambda= \t{ \mat\Lambda}$, which is denoted by $\Lambda$ used in the remaining part of this section.
Even in this simplest case, there are 5 types of fixed points, the locations of which are visualized
in the 3-dimensional space $( P, q, r)$ shown in Figure \ref{fig:d1}(a).
Each type of the fixed points has an intuitive meaning in terms of the two-player game between
$\calG$ and $\calD$.
We list the detailed information in Table \ref{tab:fixed-points},
in which we  define  a function 
$ %\[
\beta(\tau) = \begin{cases}
[1+ (\tfrac{\Lambda}{2}-\tfrac{\Lambda}{\tau})^{-1}]^{-1}, &\text{if } \tau\leq \frac{2\Lambda}{\Lambda+2}\\
+\infty, &\text{otherwise}
\end{cases}
$.%\]
%which is needed in specifying the stable region for each type of fixed points.
\vspace{-.8em}
\paragraph{Phase diagram.}
By analyzing the local stabilities of these fixed points, we obtain the phase diagram as shown in Figure \ref{fig:d1}(b). (The details can be found in the Supplementary Materials.) In particular, three major phases are identified under different settings of the learning rates $\tau$ and $\ttau$.

\emph{Noninformative phase:} We say that the ODE \eqref{eq:PCA-ODE} is in a noninformative phase if either a type-1 or type-2 fixed point in Table \ref{tab:fixed-points} is stable. In this case,   $P_t$ can be trapped at zero, which indicates that the generator's parameter vector $\mV$  has no correlation with the true feature vector $\vu$. 
 In Figure \ref{fig:d1}(b), the region labeled as noninfo-1 is the stable region for the type-1 fixed point, and noninfo-2 is 
the stable region for the type-2 fixed point. The two regions have no overlap. However, we note that 
in noninfo-1, the type-3 fixed points can also be stable, in which case the stationary point of the ODE is determined by the initial condition.

\emph{Informative phase:} We say that the ODE \eqref{eq:PCA-ODE} is in an informative phase if neither  type-1 nor type-2 fixed point is stable, and if at least one fixed point of type-3 and type-5 is stable. In this case, it is guaranteed that $P$ is nonzero, indicating that the generator can achieve non-vanishing correlation with the real feature vector. In addition, the stable regions for the type-3 and type-5 fixed points are disjoint. They are shown in Figure \ref{fig:d1}(b) as info-1 and info-2, respectively. The difference between the two region is that, in info-1,   $q$ is exactly $0$ indicating that the discriminator is completely fooled, whereas  in info-2, $q$ is nonzero. 

\emph{Oscillating phase:} We say that the ODE \eqref{eq:PCA-ODE} is in an oscillating phase if none of  the fixed points  in Table \ref{tab:fixed-points} is  stable.
In this phase, limiting cycles emerge and the system will oscillate on these cycles indefinitely.
Moreover, we found two types of limiting cycles. 

To further illustrate the phase transitions, we draw 4 phase portraits
in Figure \ref{fig:d1} corresponding to different choices of the step sizes. The figures in the middle two columns show the two types of limiting cycles that can emerge in the oscillating phase. 

When $d>1$, the situation in the Info-1 phase is same. In particular, the red line between Info-1 and Noninfo-1 in Figure \ref{fig:d1}.(a) is determined by the left inequality in \eqref{eq:con}. The blue line between Info-1 and oscillating phases is governed by the right inequality in \eqref{eq:con}. This explains why  the right inequality in \eqref{eq:con} is violated, the system start to oscillate. Currently, we are not able to fully characterize what happens in Info-2 when $d>1$. Simulations and the ODE's solution  shows that Info-2 will become oscillating or  even chaotic. %See the appendix for more numerical results. 

\begin{table*}[t]
\vspace{-1.7em}
\caption{\label{tab:fixed-points}List of the fixed points of the ODE
\eqref{eq:PCA-ODE} when $d=1$ and ${\Lambda}=\t{{\Lambda}}$.}
\centering{}%
\vspace{0.5ex}
\begin{tabular}{>{\centering}m{0.7cm}>{\centering}m{2.5cm}>{\centering}m{2.9cm}>{\centering}m{4cm}>{\centering}m{4.5cm}}
\hline 
Type & Location & Existence& Stable Region & Intuitive Interpretation\tabularnewline
\hline 
\hline 
1 & $ P=q=0$, $r=0$ & always &  
$  \tau > \Lambda^{2}$,  $\tfrac{\ttau}{\tau}<\tfrac{\tau+\Lambda}{\Lambda}$ 
& Both $\calG$ and $\calD$ fail, and they are uncorrelated\tabularnewline
\hline 
2 & $ P=q=0$ $r=\pm r^\ast\neq0$ 
& $\tfrac{\ttau}{\tau}\geq\tfrac{\tau+\Lambda}{\Lambda}$ or $\tfrac{\ttau}{\tau}\leq 1-\tfrac{\tau}{2}$
& 
$\max\{ 2,\tfrac{\tau+\Lambda}{\Lambda}\} \leq \tfrac{\ttau}{\tau}\leq \beta(\tau)$ 
& Both $\calG$ and $\calD$ fail, and they are correlated\tabularnewline
\hline 
3 & $q=r=0$ $ \abs{P} \in (0,1]$ & always 
& 
$\abs{P}=1$ is stable if 
$\tfrac{\tilde{\tau}}{\tau}\leq\min\{\tfrac{2\tau}{\Lambda},\max\{\tfrac{\tau^{2}\Lambda^{-1}}{\abs{\tau-\Lambda}},4\}\}  $
& $\calG$ wins and $\calD$ loses 
\tabularnewline
\hline 
4 & $ P=r=0$ $q = \pm P^\ast\neq 0$ 
& always
& always unstable & $\calG$ loses and $\calD$ wins\tabularnewline
\hline 
5 & None of $P$, $q$ or $r$ is zero 
&  not always, at most 8 fixed points
&  can be computed numerically
& Both $\calG$ and $\calD$ are informative
\tabularnewline
\hline 
\end{tabular}
\vspace{-1.5em}
\end{table*}



\begin{figure*}[t]
\center
\subfloat[] { \includegraphics[scale=0.33]{figures/space-crop}  \hspace{1.7em}}
\subfloat[] { \includegraphics[scale=0.7]{figures/gan_qt_3_3_tau_1_0_1-crop}   }
\subfloat[] { \includegraphics[scale=0.7]{figures/gan_qt_3_3_tau_1_0_5-crop}  }
\subfloat[] { \includegraphics[scale=0.7]{figures/gan_qt_3_3_tau_1_1_5-crop}  }
\subfloat[] { \includegraphics[scale=0.7]{figures/gan_qt_3_3_tau_1_2-crop}}
\vspace{-1.2em}
\\
\subfloat[] {  \includegraphics[scale=.7]{figures/phase-diagram}  \hspace{-1em}}
\subfloat[] { \includegraphics[scale=0.7]{figures/c1_wgan_pqi_4_tau0_03-crop} \hspace{.5em}}
\subfloat[] { \includegraphics[scale=0.7]{figures/c1_wgan_pqi_7_tau0_2-crop} \hspace{.5em}}
\subfloat[] { \includegraphics[scale=0.7]{figures/c1_wgan_pqi_9_tau0_4-crop} \hspace{.5em}}
\subfloat[] { \includegraphics[scale=0.7]{figures/c1_wgan_pqi_12_tau0_47-crop} } 
\vspace{-.5em}
\caption{\label{fig:d1}
(a): The locations of the five types of fixed points of the ODE \eqref{eq:PCA-ODE}. Their properties are listed in Table 1. 
%
(b)--(e): Macroscopic dynamics of Example \ref{ex:PCA} with $d=1$. The colored dots
show the experimental results of a single trial of the training algorithm and the black curves under the dots are theoretical predictions given by the ODE \eqref{eq:PCA-ODE}. The red, blue and yellow dots represent $ P_t$, $ q_t$, and $ r_t$, respectively. We set a fix the discriminator's learning rate $ \tau=0.3$ and vary the generator's learning rate $  \ttau$.
In (b),  $\ttau=0.1$.
The training process ends up in the phase of Info-1 where $\calG$ wins and $\calD$ completely
loses. In (c), $  \ttau=0.2$. It reaches a state oscillating around
the state of the experiment in (b).  In (d), $  \ttau=0.4$. It reaches
a different type of oscillatory state where $\calG$ and $\calD$ are highly correlated.
In (e), $\ttau=0.47$. The training process reaches a stationary phase of Info-2 in which both $\calG$ and $\calD$ have some correlations with the true feature vector.
%
(f): The phase diagram for the stationary state of the ODE \eqref{eq:PCA-ODE}. The colored lines illustrate the theoretical prediction of the boundaries between the different phases. Simulations results for a single numerical experiment are also shown to illustrate the oscillating phase: Each grey square represents the value of
$\frac{1}{200}\int_{800}^{1000} [(P_t - \langle P_t \rangle)^2 + (q_t - \langle q_t \rangle)^2 + (r_t - \langle r_t \rangle)^2]\dif t$ where $ \langle P_t \rangle=\frac{1}{200}\int_{800}^{1000} P_t \dif t$, and  
$\langle q_t \rangle$ and $ \langle r_t \rangle$ are defined similarly. Note that the above quantity measures the variation (over time) of the training process as it approaches steady states. 
We see that the variation is indeed nonzero in the oscillating phase (see (h) and (i) ), whereas the variation is close to zero in all other phases. 
%
(g)--(j): Phase portraits in the informative phase and the oscillating phase as projected onto the $p$--$q$ plane.
We set $ \tau=0.3$ and
increase $ \protect \ttau=0.03,\;0.2,\;0.4,\;0.47$ from left to right. These parameter settings are marked by the four red dots in the phase diagram in (f).
Figure (g) shows a case in the phase of info-1, where a subset of type (3) fixed points  are stable. Figure (h) and (i) are in the oscillating phase, and (j) is in info-2, where the fixed points of type-5 are stable.
The blue dots in the figures show the stable fixed points.
}
\vspace{-1em}
\end{figure*}

